The Interplay of Task Success and Dialogue Quality: An in-depth Evaluation in Task-Oriented Visual Dialogues

When training a model on referential dialogue guessing games, the best model is usually chosen based on its task success. We show that in the popular end-to-end approach, this choice prevents the model from learning to generate linguistically richer dialogues, since the acquisition of language proficiency takes longer than learning the guessing task. By comparing models playing different games (GuessWhat, GuessWhich, and Mutual Friends), we show that this discrepancy is model- and task-agnostic. We investigate whether and when better language quality could lead to higher task success. We show that in GuessWhat, models could increase their accuracy if they learn to ground, encode, and decode also words that do not occur frequently in the training set.

==> discussion_v2.tex <==
\section{Discussion}
\label{sec:discussion}

%We wonder whether this issue due to the different properties of
 % the dialogue generated during inference compared to the human
 % dialogues the model has seen at training time

%our analysis showed that, when the
 % Guesser is updated at every turn, the performance is stable across
  %the dialogue turns both for GuessWhich and GuessWhat. This
  %phenomenon is not due to the simple LSTM architecture both ReCap and
  %GDSE are using to encode the dialogue history, because even the
 % Hierarchical Recurrent Encoder-Decoder architecture of Diverse shows
  %the same behaviour. Is this issue due to the different properties of
  %the dialogue generated during inference compared to the human
  %dialogues the model has seen at training time? What is the per-turn
  %performance of GDSE-CL and GDSE-Mixed-Batches, which are trained
  %also on generated dialogues? Interestingly, GDSE-CL shows a
  %considerable increase compared to GDSE-SL but it is not clear where
  %this boost come from. See the Bengio paper on this.}

\begin{figure*}[t]\centering \hspace*{-0.1cm}
	\begin{tabular}{ll}
		\includegraphics[scale=0.3]{images/accuray_human_len.pdf} &
		\includegraphics[scale=0.3]{images/num_distractor_and_rare.pdf}
	\end{tabular}
	\caption{The length of human dialogues is a proxy of the difficulty of
		the game: what is easy/hard for humans is easy/hard for models
		(\textbf{left}); longer human dialogues contain more
                rare words, more distractors and
		more distractors of the same category of the target object (\textbf{right}).} %25 (ReCap), 35 SL + 25 CL (GDSE-CL), 5 (DynoNet)
	\label{fig:lenght}
	\vspace*{-10pt}
\end{figure*}

Before concluding the paper, we would like to give a glance to
how models and human relates with respect to difficulty of games.
  %Before concluding the paper, we would like to bring attention on an
  % underestimated issue that should be further investigated to
  % understand%
  % models behaviour, namely the role of ``rare words'' in referential
  % dialogues.  As sample, we have examined GuessWhat?! dialogues.

First of all, as shown in Figure~\ref{fig:lenght} (left), the length
of the dialogue produced by humans while playing the game is a good proxy of its
difficulty: the longer is the human dialogue, the lower is the
accuracy the model
reaches for that game (blue bars).  Interestingly, generated dialogues show a similar result across games of different difficulty: their TS is
around 9\% lower than those reached by processing human dialogues (the blue vs red bars) independently of the
length of the game, i.e., the difficulty of the game. A second important
observation is illustrated in Figure~\ref{fig:lenght} (right) which
shows that games for which humans ask a higher number of questions
are about images with a higher number of distractors and with a
higher number of distractors of the same category of the
target. Thirdly, more than half (55\%) of the words in the vocabulary
are ``rare'',  i.e., they are used less than 15 times in the training
set;  most of these rare words are
nouns (79\%) or verbs (11\%).  In 10\%
of the games in the test set humans have used at least one rare word and
the accuracy on these games is rather low: -10.88\% than the overall
accuracy. These dialogues are longer than the ones not containing
``rare'' words (resp., 7.80 vs. 4.7 turns in average).
% and models
%accuracy on them is rather low (-10.88\% than the overall accuracy),
%the rare words are on average used at turn 5.48 and most of them are
%nouns (79\%) or verbs (11\%).


%\begin{table}
%\centering
%\begin{tabular}{l|ll}\toprule
% & Games with rare words & Game without rare words\\\midrule
%Percentage of games & 10\% & 90\%\\
%Lenght of human dialogues & 7.80 & 4.77\\
%Turn with rare words & 5.48 & NA\\
%Task Accuracy & 38.41 & 49.29\\\bottomrule
%\end{tabular}
%\caption{GDSE-SL (GuessWhat?! test set games): Analysis of games
 % containing ``rare'' words} \label{tab:rare}
%\end{table}

Putting together these observations, we conjecture that current models
fail to properly ground and use \emph{rare words}. This weakness could
be behind the main finding reported in our experiments, namely that the learning TS curve increases pretty quickly
after a few epochs even when trained on small datasets and stay rather
flat afterwords. 
Figures~\ref{fig:sample} shows some samples of games
in which humans have used a rare word, it illustrates the  human
vs.\ generated dialogue and whether the model succeeds in guessing the target object
when receiving the former or the latter. The example on top, shows that
if the model fails to generate an appropriate word (e.g.\ the rare word
``\emph{pancake}'') this can have a domino effect on the next words
and the next questions it generates. Furthermore, the model can fail
encoding rare words, (e.g., ``'\emph{macbook}'' in
Figure~\ref{fig:sample}-bottom). The failure in encoding human questions
containing rare words should be kept in mind when comparing 
model performance on human dialogues vs. generated dialogues since the
latter might contain mistakes by the Oracle and the decoder that could
be misleading or not informative, but the
latter might contain rare words that could also be
misunderstood.\footnote{We have compared models' performance when taking
as input human vs.\ generated dialogues; in the former case, the
decrease in the accuracy  correlates with the number of rare words 
used by the questioner -- even when comparing games with equal number
of distractors; moreover, the difference of the accuracy reached by
the model in the two settings is higher when comparing games for which
humans have used a higher number of rare words.}



%\begin{wrapfigure}{R}{0.48\textwidth}
\begin{figure*}[t]
	\centering
	\begin{minipage}{3cm}
		\includegraphics[width=3cm]{images/panckcake_target.png} 
	\end{minipage}
	\begin{minipage}{9cm}\small
		\begin{tabular}[t]{l@{\hspace{-0.2cm}}r|l@{\hspace{-0.2cm}}r}
			\multicolumn{2}{c}{Human dialogues} & \multicolumn{2}{c}{Generated dialogues}\\
			\bf Questioner & \bf Answerer & \bf Questioner & \bf Answerer\\[3pt]
			1. Is it a man? & No & 1. Is it a person? & No\\[3pt]
			2. Is it food?  & Yes & 2. Is it food? & Yes\\[3pt]
			3. Is \emph{pancake}?  & No & 3. Is it pizza? & Yes \\[3pt]
			4. Is egg? & Yes & 4. Is it the pizza in front? & Yes\\[3pt]
			&  & 5. \ldots & \\
			\multicolumn{2}{l}{\bf $\leadsto$ model suceeds guessing} &
			\multicolumn{2}{l}{\bf
				$\leadsto$
				model
				fails guessing} \\
		\end{tabular}
	\end{minipage}
	\vspace*{.6cm}

	\begin{minipage}{3cm}
		\includegraphics[width=3cm]{images/macbook_target.png} 
	\end{minipage}
	\begin{minipage}{9cm}\small
		\begin{tabular}[t]{l@{\hspace{-0.2cm}}r|l@{\hspace{-0.2cm}}r}
			\multicolumn{2}{c}{Human dialogues} & \multicolumn{2}{c}{Generated dialogues}\\
			\bf Questioner & \bf Answerer & \bf Questioner & \bf Answerer\\[3pt]
			1. Is it the cat? & No & 1. Is it the cat? & No\\[3pt]
			2. Is it the \emph{macbook}?  & Yes & 2. Is it the laptop? & Yes\\[3pt]
			3. The whole thing?  & Yes & 3. Is it the whole laptop? & Yes \\
			 4. & & \ldots &\\
			\multicolumn{2}{l}{\bf $\leadsto$ model fails guessing} &
			\multicolumn{2}{l}{\bf
				$\leadsto$
				model
				succeeds guessing} \\
			%1. Is it the cat? & No & &\\[3pt]
			%2. Is it the laptop?  & Yes & &\\[3pt]
			%3. Is it the whole laptop?  & Yes & &\\
			%\ldots &  & & \\
			%\multicolumn{2}{l}{\bf $\leadsto$ model succed guessing}
		\end{tabular}
	\end{minipage}\caption{Examples of GuessWhat games in which humans use 'rare' words (rare words in italic) and the corresponding generated dialogues. }\label{fig:sample}
	\vspace*{-.3cm}
\end{figure*}



%\tb{dialoghi in training diversi da dialoghi in
 % testing. Ripetizioni.. il modello fa casino.}


%In the Seq2Seq architecture, the encoder is designed to learn to
%capture natural language meaning by building embeddings that ground
%text into vision. The decoder instead is driven puerly by the
%probability distribution of words. As such, it tends to use only very
%frequent words. We have compared the Zipf's curve of human dialogues
%generated to play the games in the training set with the dialogues
%generated by the XX model when playing the same games. Whereas human
%dialogues respect the Zipf's law, models dialogue do not.

%\tb{Zipf's law: the frequency of a word is inversely proportional to its rank in
 % the global list of words after sorting by decreasing frequency.}

%This drastic difference raises the question of whether the poverty of
%language of models contributes to their lower performance compared to
%humans. Hence, we have cluster dialogues based on the presence of
%``rare'' words and inspection them.

%\tb{accuracy}

%\tb{alaysis of dialoguee}
%\begin{figure}[t]\centering 
%\begin{tabular}{c}
%\includegraphics[scale=0.35]{images/zipf} 
%\end{tabular}
%\caption{Zipf'law } \label{fig:zipf}
 % \vspace*{-10pt}
%\end{figure}



%\rb{Novel questions: but is really good?}

%\tb{Difference due to dataset size impact of NLG diversity --
 % stability vs diversity}

%\rb{Linguistic Metrics: quality of the question but in isolation. Imp:
%question coherence/consistenty, informativiness. All models show
%inconsistency, the answerers answers in inconsistent way. Cite work on
%inconsistency~\cite{marg:dont19,ray-etal-2019-sunny}}


%\tb{\cite{khandelwal-etal-2018-sharp} show that NN LM are able to use
 % 200 tokens of context on average. sensiste to word order withing the
 % most recent sentences but ignores it in byond 50
  %tokens. \cite{sank:done19} show NN do not take dialogue histhory
 % into account. 

%\tb{\cite{wu-etal-2019-self}: methods to take histhory
 % into account more. }




==> experiments_v3.tex <==
\section{Experiments and Results}
\label{sec:experiments}

As a preliminary analysis, we have compared humans and models by
looking at their task success (TS) and the quality of their dialogues
in the three games GuessWhich, GuessWhat?! and MutualFriends. 
We have
evaluated all the models described above, in their supervised,
cooperative or reinforcement learning version, for each tasks aiming to
test whether some pattern can be found irrespectively of the model and
data explored.  Our results confirm
what has been shown in~\cite{shekhar-etal-2019-beyond} for
GuessWhat?!: task success (TS) does not correlate with quality of
dialogues: models with similar TS generate dialogues which vary
quite a lot with respect to the linguistic metrics. Our comparative
analysis shows that this discrepancy is not due to a specific dataset
nor to a specific architecture or to a specific learning
paradigm. Detailed results are reported in the Supplementary
Material. Here, we focus on understanding the learning process of
these two skills at the core of referential games: guessing the
referent and asking good dialogues.


\subsection{Comparison Across the Epochs and by
  Downsizing the  Training Set}
%Since TS and dialogue quality are two crucial components of the
%evaluation of task-oriented dialogues and we have seen that there is
%no correlation between them, we are interested in understanding their
%relation. 
In this experiment, we study the interplay between TS and
LD  across epochs and by varying the size of the
training data.  For each task, we consider the best performing model on
that task trained with supervised learning (SL) since the other
learning paradigms build on these SL epochs. Hence, we focus on
ReCap, GDSE-SL and DynoNet.
%, and wonder for \emph{how long} (in terms of
%epochs) a model should be
%trained to reach a good balance between the two types of
%metrics. 

%\begin{wrapfigure}{L}{0.60\textwidth}
%\begin{center}
\cut{
\begin{figure}[t]\centering \hspace*{-0.1cm}
\includegraphics[scale=0.35]{images/all_tasks_summary_3.pdf}
%\end{center}
\caption{Comparison of Task Success (TS) and Linguistic
  Divergence (LD) for GDSE-SL (GuessWhat?!), ReCap (GuessWhich),
  DynoNet (MutualFriends) and Humans LD lower-bound metric in
  yellow. The LD of the generated dialogues keeps decreasing (moving
  close to human level) while  high TS is reached after few
  epochs marked by the colored circles in the curves.} %25 (ReCap), 35 SL + 25 CL (GDSE-CL), 5 (DynoNet)
\label{fig:summary}
  \vspace*{-10pt}
\end{figure}
%\end{wrapfigure}
}

\cut{
	\begin{wrapfigure}{R}{0.5\textwidth}
		%\begin{center}
		%\begin{figure}[t]\centering \hspace*{-0.1cm}
		\includegraphics[scale=0.37]{images/all_tasks_summary_3.pdf}
		%\end{center}
		\caption{Comparison of Task Success (TS) and Linguistic
			Divergence (LD) for GDSE-SL (GuessWhat?!), ReCap (GuessWhich),
			DynoNet (MutualFriends) and Humans LD lower-bound metric in
			yellow. The LD of the generated dialogues keeps decreasing (moving
			close to human level) even though we no longer notice improvements in TS, whose highest value is reached well before.} %25 (ReCap), 35 SL + 25 CL (GDSE-CL), 5 (DynoNet)
		\label{fig:summary}
		\vspace*{-10pt}
		%\end{figure}
	\end{wrapfigure}
}


\begin{figure}[t]
	\centering \hspace*{-0.1cm}
	\includegraphics[width=0.8\linewidth]{images/all_tasks_summary_3.pdf}
	%\end{center}
	\caption{Comparison of Task Success (TS) and Linguistic
		Divergence (LD) for GDSE-SL (GuessWhat?!), ReCap (GuessWhich),
		DynoNet (MutualFriends) and Humans LD lower-bound metric in
		yellow. The LD of the generated dialogues keeps decreasing (moving
		close to human level) even though we no longer notice improvements in TS, whose highest value is reached well before.} %25 (ReCap), 35 SL + 25 CL (GDSE-CL), 5 (DynoNet)
	\label{fig:summary}
	\vspace*{-10pt}
\end{figure}

To understand \emph{how long} a SL model has to be trained to reach
its best performance, we compare the TS (MPR for GuessWhich and ACC
for the other two tasks) and LD metrics obtained by ReCap, GDSE-SL and
DynoNet when trained on the full datasets of GuessWhich, GuessWhat?!
and MutualFriends, respectively. 

As we can see from
Figure~\ref{fig:summary}, the highest TS is reached earlier in
GuessWhich and in MutualFriends than in GuessWhat?!, which suggests
that GuessWhat?! is a more challenging referential game.  More
interestingly, for all the tasks, the LD of the generated dialogues
keeps decreasing (moving close to human level) 
even though we no longer notice improvements in TS, whose highest value is reached well before.  Figure~\ref{fig:epochs-datasize} reports
the details of  the most salient  linguistic metric: we see that for all the
tasks across the epochs a high entropy is reached already after a few
epochs; this means that though the number of words used is
small, models learn to distribute their use well; all the other metrics instead improve through the
epochs quite a lot. 

\textbf{Results} All in all, this first analysis shows that
generating a linguistically rich dialogue is a harder task than
learning to play a guessing task. This result holds in all cases
despite the target being an entity in a graph described by
linguistic attributes (MutualFriends), an object (GuessWhat?!) or an
image (GuessWhich).  This unexpected behaviour suggests that the best model
of a task-oriented system should not be chosen by looking at the task
success only. Even more interestingly, it also shows that the model
does not take advantage of its improved linguistic skills to perform
better on the game. We come back to this observation in the next
experiments.
\begin{figure*}[t]\centering 
	%\begin{tabular}{c}
	\includegraphics[width=1\linewidth]{images/all_tasks_focus_2.pdf} 
	%\includegraphics[scale=0.2]{images/Guesswhat_epoch}\\
	%\end{tabular}
	\caption{Comparison across epochs 
		and by downsizing the training data using the metrics
                described above: Task Success (TS), Games with Repeated Questions (GRQ), Mutual
                Overlap (MO), unigram entropy (H) and Global Recall
                (GR); all metrics are scaled between 0 and 1 (y-axis).
               \textbf{Left:} GDSE-SL on
		GuessWhat?!. \textbf{Middle}: ReCap on
		GuessWhich.  \textbf{Right}: DynoNet on MutualFriends. Downsizing
		the training data has a higher impact, both for TS and some
		linguistic metrics,  in GuessWhat?! than in GuessWhich. Among the linguistic metrics,
		entropy is the most stable and GR increases through
                the epochs in all tasks. The dataset of MutualFriends
                is too small to analyse the effect of downsizing it.} \label{fig:epochs-datasize}
	\vspace*{-10pt}
\end{figure*}


%To report the
%comparison within the same graph, we normalize the metrics w.r.t. to
%human values (1 very far from human and 0 equal to human for MO and
%GRQ, vice-versa for NQ).
%\footnote{For readability, in
 % Fig.~\ref{fig:epochs-datasize} we do not report the Recall metrics:
  %they follow the same patterns of the others.} 

%Finally, the fact that the model does not reach the global
%recall of humans and \rb{that its local recall is far from 100\%, show
%  that xxxx.} 


To understand \emph{how much} a model should be trained on a task, we
compare models trained on data sets of decreasing size. We have
evaluated the models by training them with 50\% and 25\% of the
standard GuessWhat?! and GuessWhich datasets. For MutualFriends, we
have not run the downsizing analysis since the dataset is too small.
For readability reason, in Figure~\ref{fig:epochs-datasize} we report
only the results obtained with the 25\% setting since they represent the
observed pattern well enough. The y-axis reports the metrics scaled
between 0 and 1.

In GuessWhich the TS (yellow lines) does
not decrease by downsizing the dataset: when using just the 25\% of
the full dataset (dotted line) it gets very close to the highest MPR
obtained by the model trained on the full dataset (solid line) already
after the first 5 epochs. Interestingly, the linguistic metrics do not
get worse- with the only exception of GR. Instead, the TS reached in GuessWhat?!
decreases when downsizing the training data (again, yellow solid
vs. dotted lines) and dialogues quality is affected too (with the
exception of entropy and GR). \textbf{Result} The discrepancy between
task success and quality of dialogues is observed also when downsizing
the training data. Moreover, GuessWhat?! results to be 
a harder referential game than GuessWhich as commented above.
%Surprisingly, the model trained on less data is the one with
%more novel questions (blue dotted line). This is a rather interesting
%result that deserves further investigation. We conjecture that being
%trained on a large amount of data is beneficial for reaching
%``stability'' of the model, which is usually considered a plus, but
%within the natural language generation task ``stability'' may lead to
%lack of novelty and linguistic creativity.


%\at{Per questa sezione abbiamo D-SL per 2c) ma non per 2d). D-CL non riusciamo a replicarlo. Per Guesswhat GDSE-SL abbiamo 2c) e 2d) per 100\% e 50\% - manca 25\%.}




\cut{SM: \begin{figure}[t]\centering 
\begin{tabular}{c}
%\includegraphics[width=\columnwidth]{images/fig2_compressed.pdf}\\
\includegraphics[width=\columnwidth]{images/VD_diverse_chart}\\
\end{tabular}
\caption{Diverse-SL: comparison across epochs.}\label{fig:epochs_d_sl}
  \vspace*{-10pt}
\end{figure}
}

%\begin{figure}[t]\centering 
%\begin{tabular}{c}
%\includegraphics[width=\columnwidth]{images/fig2_compressed.pdf}\\
%\includegraphics[width=\columnwidth]{images/GW_chart}\\
%\end{tabular}
%\caption{GDSE-SL: comparison across epochs 
 % and by downsizing the training data. Best accuracy marked with a yellow diamond. }\label{fig:epochs_gdse_sl}
%  \vspace*{-10pt}
%\end{figure}

%\at{The results of Guesswhat D-SL are reported in figure~\ref{fig:epochs_d_sl}.
%The results of Guesswhat GDSE-SL are reported in
%figure~\ref{fig:epochs_gdse_sl}.} 


%\subsection{Experiment3: a screen shot of the languages through the
%  Zipf's law}

%The highest TS is reached earlier in GuessWhich and in MutualFriends
%than in GuessWhat?!  and downsizing their training sets does not have
%a big impact on the performance reached by the models, this suggests
%that GuessWhat?! is a more challenging referential game. On the other
%hand, the size of the training data has an impact on the quality of
%the GuessWhich dialogues generated by models wheras does not alter
%those of the GuessWhat?! games. 


From the results of this first experiment, it emerges fairly clearly that in all
referential games we have considered, models learn to perform well on
the task quite quickly. Little is gained by keeping on training them
with more epochs even though the quality of the dialogues increases.
We wonder \emph{why models are not able to profit from such increase of 
language performance}. In the following, we try to understand
whether the reason can be found in how the encoder exploits the
dialogue history or in the mistakes made by the decoder in generating
questions or by the Oracle in answering them.

\subsection{Is the Encoder behind the Failure of the Models to Exploit a better Language Performance?}

By using data perturbation, it has been shown that neural networks
(NNs) language models are
capable of using context consisting of about 200 tokens on average, but
they have more difficulty in modeling tokens beyond the first nearest
50th positions~\cite{khandelwal-etal-2018-sharp}. By applying a
similar analysis, Sankar et al. \shortcite{sank:done19} have shown
that NN conversational agents are not able to take the dialogue
history into account. We wonder whether this can be the reason behind
the failure of the models to exploit a better language proficiency.

%Hence, even if the number of informative
%questions within the dialogue would increase through the epochs, maybe
%the models would not be able to exploit them.  
To this end, we run a by-turn evaluation checking whether the
information incrementally gained through the dialogue brings an
increased performance. We consider the two asymmetric guessing games,
GuessWhich and GuessWhat?!, whose dialogues are based on turns.  Again,
we evaluate the two best performing supervised models, viz.\ ReCap and
GDSE-SL. The performance of ReCap is flat across the dialogue turns,
confirming results reported in \cite{mura:impr19} for other
models. Instead, the performance of GDSE-SL keeps on increasing at
each turn from the beginning till the end of the dialogue though the
increase in the first 3 turns is higher than in later ones.  This
seems to suggest that in GuessWhat?!, models accumulate information
through the dialogue to some extend. We believe the differences
between ReCap/GuessWhich and GDSE-SL/GuessWhat?! is due to crucial
differences in the dataset designs. As it has been highlighted in
Testoni et al. \shortcite{test:thed19}, in GuessWhich the image
caption is already quite informative to retrieve the target image, the
evaluation metric is rather coarse and, as stated in Zhou et
al. \shortcite{zhou:buil19}, the candidate images are quite diverse
from each other. On the other hand, in GuessWhat?! the same image is
associated with different target objects, the evaluation metric is
more fine-grained, and the similarity between candidate objects differ
across the games.  \textbf{Result} GDSE-SL manages to
use information incrementally received through the dialogue, this
means that its
encoder manages to model the dialogue history to some extent, still
it fails to exploit better language proficiency to reach higher task
success. These observations suggest that failure of models
in exploiting a better quality of dialogues \emph{is not} due to the
lack of the encoder to represent the dialogue history.

\subsection{Are the Decoder or the Oracle behind the Failure of the Models to exploit a better Language Performance?}

In the literature on GuessWhat?! and GuessWhich, attention has been
so far put only on the Q-Bot; as a consequence, the
A-Bot is usually frozen through the epochs. Wrong answers by the A-Bot could provide even
inconsistent information as shown in Li et
al. \shortcite{marg:dont19}; Ray et
al. \shortcite{ray-etal-2019-sunny}. Hence, the mistakes coming from the A-Bot could
prevent the Q-Bot reaching a higher performance. For instance, the
Oracle commonly used for GuessWhat?! has an accuracy of around 80\%,
which means there is a 83\% probability that an 8-turn generated
dialogue contains at least one wrong answer, but not much  is known
about its impact. Similarly, the TS could be influenced by the
model having asked ``wrong'' questions.

To better understand the impact of the mistakes made by the decoder or
by the A-bot, we
have evaluated ReCap and GDSE-SL across the epochs on the dialogues asked
by humans for test set games. The same TS pattern has emerged: the
models reach a high TS pretty quickly (around epoch 30 for GDSE-SL and
around epoch 25 for ReCap). \textbf{Result} This suggests that the difficulty of the
models to exploit an higher linguistic proficiency most probabily \emph{is not} due to the
mistakes made by the A-bot nor to the failure of the decoder in
generating good questions. 


